Quantification and Aggregation over Concepts of the Ontology

We argue that in some KR applications, we want to quantify over sets of concepts formally represented by symbols in the vocabulary. We show that this quantification should be distinguished from second-order quantification and meta-programming quantification. We also investigate the relationship with concepts in intensional logic. We present an extension of first-order logic to support such abstractions, and show that it allows writing expressions of knowledge that are elaboration tolerant. To avoid nonsensical sentences in this formalism, we refine the concept of well-formed sentences, and propose a method to verify well-formedness with a complexity that is linear with the number of tokens in the formula. We have extended FO(.), a Knowledge Representation language, and IDP-Z3, a reasoning engine for FO(.), accordingly. We show that this extension was essential in accurately modelling various problem domains in an elaboration-tolerant way, i.e., without reification.

==> deprecated/old_sections/0.abstract2.tex <==
\begin{abstract}

%In first-order logic (FO), quantifications range over sets of elements of the domain.
%Such quantifications allow FO to express knowledge more concisely than propositional calculus can.  
%Similarly, Second Order (SO) logic is more expressive than FO thanks to its quantification over relations and functions.

%The first phase of developing an intelligent system is the selection of an ontology of symbols representing relevant concepts of the application domain.
%These symbols are then used to represent the knowledge of the domain.
%This representation should be \emph{elaboration tolerant}, in the sense that it should be convenient to modify it to take into account new knowledge or requirements.
%Unfortunately, current formalisms require a significant rewrite of that representation when the new knowledge is about the \emph{concepts} themselves: the developer needs to ``\emph{reify}'' them.
%This happens, for example, when the new knowledge is about the number of concepts that satisfy some conditions.
%The value of expressing knowledge about concepts, or ``intensions'', has been well-established in \emph{modal logic}.
%However, the formalism of modal logic cannot represent the quantifications and aggregations over concepts that some applications need.
The power of a  KR language for compact expression of knowledge lies for an important extent in the way it allows us to abstract over certain types of objects, e.g., to quantify, count,  sum, \dots over them. In this paper, we argue that in some KR applications, we want to abstract  over sets of {\em concepts} formally represented  by symbols in vocabulary. We show this should be distinguished from second order quantification and meta-programming quantification. We investigate the relationship to concepts in intensional logic. Finally, we present an extension of First order logic to support this and show that in this case, a more elaboration tolerant theory is obtained.

%To address this problem, we developed an extension of first order logic that allows referring to the \emph{intension} of a symbol, i.e., to the concept it represents.  
%We implemented this extension in IDP-Z3, a reasoning engine for FO($\cdot$) (aka FO-dot), a knowledge representation language that integrates classical logic and logic programming.
%This extension makes the formalism more elaboration tolerant, but also introduces the possibility of syntactically incorrect formula.
%Hence, we developed a guarding mechanism to make formula syntactically correct, and a method to verify correctness.  
%The complexity of this method is linear with the length of the formula.

%This paper describes these extensions, how their relate to intensions in modal logic and other formalisms, and how they allowed representing the knowledge of four different problem domains in an elaboration tolerant way.  


\end{abstract}


\ignore{
    ** old version
    
    %In first-order logic (FO), quantifications range over sets of elements of the domain.
    %Such quantifications allow FO to express knowledge more concisely than propositional calculus can.  
    %Similarly, Second Order (SO) logic is more expressive than FO thanks to its quantification over relations and functions.
    
    This paper focuses on quantifications whose nature, we believe, is generally undervalued within the Knowledge Representation community: they range over a set of \emph{concepts}, i.e., of \emph{intensional objects} identified in the ontology.
    
    Hence, we extend first order logic to allow referring to the \emph{intension} of a symbol, i.e., to the concept it represents.  
    Our formalism is more elaboration tolerant than simpler formalisms that require reification, but also introduces the possibility of syntactically incorrect formula.
    We introduce a guarding mechanism to make formula syntactically correct, and present a method to verify correctness.  
    The complexity of the method is linear with the length of the formula.
    
    We also extend FO($\cdot$) (aka FO-dot), a logic-based knowledge representation language, in a similar way, and show how it helped solve practical problems.
    
    The value of expressing intensional statements has been well-established in \emph{modal logic}.
    We show how our approach expands on the understanding of intensions as studied in modal settings by, e.g., Fitting, in a way that is of value in non-modal settings as well.
}

==> deprecated/old_sections/old_stuffs/abstract.tex <==
\begin{abstract}
\mvdh{Perhaps the title can be improved: `Specifying with intension: Adding intensional objects to First-Order Logic' or something like that. (a play on words with 'intent' could be nice ;) }
%...

In First Order logic (FO), a predicate, i.e., a relation between objects in a universe of discourse, is formalized as the set of tuples of objects that are in that relation.
An important class of knowledge is knowledge about the extension of these sets; for example, knowledge that if an object belongs in set A, it also belongs in set B.
Such knowledge can be called "extensional".
In extensional knowledge, two predicates are identical if they have the same extension.  

Another important class of knowledge is knowledge about the "intension" of these predicates.  
Two predicates with the same extension may have distinct intensions.
For example, the predicates "morning star" and "evening star" have distinct intensions, even though they have the same extension, \{Venus\}.

$FO(\cdot)$ is a KR language that extends FO. In this paper, we further extend $FO(\cdot)$ to allow representation of intensional knowledge. \marc{This abstract : is not detailed enough I would say. It has been attempted before to add intensional concepts to a logic. In what is this proposal different?}

\dmar{I have rewritten the abstract - see below. I didn't replace it with the old one since they can be further mixed.}

First-order logic (FO) predicate, i.e., a relation between objects in a universe of discourse, is formalized as the set of tuples of objects. An important class of knowledge is about the extension of these sets; for example: "if an object belongs in set A, it also belongs in set B". 

It is easy to imagine situations where we would like to state some properties about the concepts rather than objects. We usually solve this problem by reifying the symbols into the objects. But it would be natural if we can speak about these concepts themselves. Furthermore, reification restricts us to the type and arity of symbols.

Talking about the meaning of the concepts gives us a clue to the intensional logic, which brings us to the class of knowledge about intensions. A long-established example would be the "morning star" and "evening star". They have different intensions (meaning), even though they both designate the same object, planet Venus.

In this paper, we integrate the idea of intensional objects into the first-order logic to abstract over similar concepts. Also, we explain the difference between higher-order logic and our approach.

\mvdh{I have also attempted a new abstract, trying to focus on 3 contributions: it's not modal logic. We explicitly differentiate between higher-order \& extensional vs intensional, and allow refering to both intension and extension. I would like to work in the different type of system (querying vs KB Paradigm) in there as well}


In first-order logic (FO), predicate symbols are generally assigned a relation over the domain, i.e. a set of tuples of values. 
The set assigned to a symbol is referred to as its \emph{extension}.% of that symbol.
An extensional logic can express knowledge such as ``all objects belonging to A also belong to B''.
In such a logic, two symbols are equal if and only if they share the same extension, and any two symbols with the same extension can be used interchangeably.
This covers an important class of knowledge.


However, one can also associate with any symbol an \emph{intension}, and while two symbols may share one and the same \emph{extension}, they can have different \emph{intension}s.
Thus, when taking into account \emph{intension}, two symbols are no longer necessarily equal if they share \emph{extension}, nor are they interchangeable.

The value of expressing intensional statements has been well-established in \emph{modal logic}; 
consider for example ``Everyone knows that Mark Twain wrote Huckleberry Finn'' and ``Everyone knows that the author of Huckleberry Finn wrote Huckleberry Finn''. 
It is easy to see that, although `Mark Twain' and `the author of Huckleberry Finn' can be used interchangeably in an extensional logic, the substitution has radically changed this sentence.

However, we show that even in a non-modal setting there is value in distinguishing between a symbol's \emph{intension} and \emph{extension}. 
For example, when one would want to count the number of properties (e.g. sneezing, coughing, ...) satisfied by an object, we are not looking to quantify over all possible sets but rather all relevant symbols in our vocabulary.
It is equally important to note that we do not want to use a higher-order formula to count the \emph{extensions} of these symbols: any property that would happen to share its extension with another would be counted only once.
By distinguishing between \emph{intension} and \emph{extension}, it becomes evident that many expressions that are generally considered within the realm of second order logic, are in fact expressions considering \emph{intension}.
\todo{as opposed to HiLog.}

In this paper, we introduce an extension on first order logic that makes this sharp distinction between a symbol's \emph{intension} and \emph{extension}, and that allows to freely refer to either when necessary, obviating the need for manual application of techniques such as reification.
We describe our implementation in a knowledge base system, and how it helped solve practical problems.






\end{abstract}

==> eptcsdata.tex <==
\providecommand{\firstpage}{213}
\providecommand{\publicationstatus}{S. Costantini, E. Pontelli, A. Russo, F. Toni,\\R. Calegari, A. D'Avila Garcez, C. Dodaro, F. Fabiano,\\ S. Gaggl, A. Mileo, (Eds.): ICLP 2023\\
EPTCS 385, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.385.22}{10.4204/EPTCS.385.22}}
\pdfoutput=1

